Search for new phenomena in final states with large jet multiplicities and missing transverse momentum at sqrt(s)=8 TeV proton-proton collisions using the ATLAS experiment

A search is presented for new particles decaying to large numbers (7 to greater or equal to 10) of jets, missing transverse momentum and no isolated electrons or muons. This analysis uses 20.3/fb of pp collision data at sqrt(s)=8 TeV collected by the ATLAS experiment at the Large Hadron Collider. The sensitivity of the search is enhanced by considering the number of b-tagged jets and the scalar sum of masses of large-radius jets in an event. No evidence is found for physics beyond the Standard Model. The results are interpreted in the context of various simplified supersymmetry-inspired models where gluinos are pair produced, as well as a mSUGRA/CMSSM model.

==> frontmatter.tex <==
\RequirePackage{lineno}
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
  \expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
  \expandafter\let\csname oldend#1\expandafter\endcsname\csname end#1\endcsname
  \renewenvironment{#1}%
     {\linenomath\csname old#1\endcsname}%
     {\csname oldend#1\endcsname\endlinenomath}}%
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}}%
\AtBeginDocument{%
\patchBothAmsMathEnvironmentsForLineno{equation}%
%\patchBothAmsMathEnvironmentsForLineno{equation*}%
\patchBothAmsMathEnvironmentsForLineno{align}%
\patchBothAmsMathEnvironmentsForLineno{flalign}%
\patchBothAmsMathEnvironmentsForLineno{alignat}%
\patchBothAmsMathEnvironmentsForLineno{gather}%
\patchBothAmsMathEnvironmentsForLineno{multline}%
}

\usepackage{atlasphysics}
%\usepackage[bf,tight]{subfigure}
\usepackage{subfig}
\usepackage{mathrsfs}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{slashed}
\usepackage{afterpage}


%\usepackage{minipage}
%\usepackage{mathabx}
% \usepackage{mcite}
\usepackage{amsmath,amssymb}
\usepackage{url}
\usepackage{textpos}
\usepackage{placeins}
%\usepackage{atlascover}

\usepackage{hyperref}
%\usepackage{hypernat}  % makes hyperref work with natbib

%\biboptions{sort,merge}

\input{susydefs}
%\graphicspath{../INT/}
\DeclareGraphicsExtensions{.pdf}

\newcommand{\mSUGRA}{mSUGRA/CMSSM}
\newcommand{\mSUGRAShortened}{CMSSM}
\newcommand{\ourpt}{p_\mathrm{T}}
\newcommand{\mT}{\ensuremath{m_{\rm T}}}
\newcommand{\anactualptmissvecwithapinit}{{{\bf p}}_\mathrm{T}^\mathrm{\,miss}}
\newcommand{\ourvecptmiss}{\ensuremath{\anactualptmissvecwithapinit}}
\newcommand{\ourmagptmiss}{{\ensuremath \MET}}
\renewcommand{\HT}{{\ensuremath{H_{\rm T}}}}
\newcommand{\metsig}{{\ensuremath{\ourmagptmiss/\sqrt{\HT}}}}
\newcommand{\rootgev}{{\ensuremath{\GeV^{1/2}}}}
\newcommand{\pthreshold}{{\ensuremath{p_{\rm{T}}^{\rm min}}}}
\newcommand{\softet}{\ensuremath{\sum \textrm{E}_\textrm{T}^\textrm{CellOut}}}
\newcommand{\softoHT}{\ensuremath{\softet/H_{\rm{T}}}}
\newcommand{\mult}{{\ensuremath{n_{\rm jet}}}}
\newcommand{\sigmamaxbsm}{\ensuremath{\sigma_{\rm BSM,max}^{95\%}  \cdot A \cdot \epsilon}}
\newcommand{\nmaxbsm}{\ensuremath{N_{\rm BSM,max}^{95\%}}}
\newcommand{\smin}{{\ensuremath{s_\textrm{min}}}}
\newcommand{\smax}{{\ensuremath{s_\textrm{max}}}}
\newcommand{\generator}[1]{\textsc{#1}}
\newcommand{\alpgen}{\generator{Alpgen}}
\newcommand{\herwig}{\textsc{Herwig}}
\newcommand{\sherpa}{\generator{Sherpa}}
\newcommand{\jimmy}{\generator{Jimmy}}
\newcommand{\prospino}{\generator{Prospino}}
\newcommand{\cteqVER}[1]{\generator{CTEQ#1}}
\newcommand{\mstwVER}[1]{\generator{MSTW#1}}
\newcommand{\nnpdfVER}[1]{\generator{NNPDF#1}}
\newcommand{\nllfastVER}[1]{\generator{NLL-fast#1}}
\newcommand{\alpgenVER}[1]{\generator{Alpgen#1}}
\newcommand{\prospinoVER}[1]{\generator{Prospino#1}}
\newcommand{\herwigppVER}[1]{\textsc{Herwig++#1}}
\newcommand{\herwigVER}[1]{\textsc{Herwig#1}}
\newcommand{\isajetVER}[1]{\generator{ISAJET++#1}}
\newcommand{\sherpaVER}[1]{\generator{Sherpa-#1}}
\newcommand{\mcatnloVER}[1]{\generator{MC@NLO#1}}
\newcommand{\acermcVER}[1]{\generator{AcerMC#1}}
\newcommand{\madgraphVER}[1]{\generator{Madgraph-#1}}
\newcommand{\pythiaVER}[1]{\generator{Pythia-#1}}
\newcommand{\msugra}{mSUGRA/CMSSM}
\newcommand{\paper}{paper}
\newcommand{\leptonic}{leptonic}
\newcommand{\Leptonic}{Leptonic}
\newcommand{\citemsugraandcmssm}{\cite{Chamseddine:1982jx,Barbieri:1982eh,Ibanez:1982ee,Hall:1983iz,Ohta:1982wn,Kane:1993td}}
\newcommand{\oursubref}[1]{{\bf (\subref{#1})}}
\newcommand{\ourtabref}[1]{table~\ref{#1}}
\newcommand{\ourfigref}[1]{figure~\ref{#1}}
\newcommand{\oursecref}[1]{section~\ref{#1}}
\newcommand{\comment}[1]{{\em[#1]}}



==> susydefs.tex <==

\newcommand{\figref}[1]{figure~\ref{#1}}
\newcommand{\figsref}[1]{figures.~\ref{#1}}
%\newcommand{\partref}[1]{part~\ref{#1}}
\newcommand{\Secref}[1]{section~\ref{#1}}
\newcommand{\tabref}[1]{table~\ref{#1}}

% susy-specific variables
\newcommand{\meff}{\ensuremath{m_{\mathrm{eff}}}} % This was an M, but all our other m's are in lower case and M_eff sticks out like a sore thumb.  So I've changed it to something more relaxing.
\newcommand{\mt}{\ensuremath{m_\mathrm{T}}}
\newcommand{\mttwo}{\ensuremath{m_\mathrm{T2}}}
\newcommand{\mc}{\ensuremath{m_\mathrm{C}}}
\newcommand{\mct}{\ensuremath{m_\mathrm{CT}}}
\newcommand{\pp}{\ensuremath{pp}}
\newcommand{\sqseight}{\ensuremath{\sqrt{s}=8}~TeV}
\newcommand{\MJ}{\ensuremath{{M_J^\Sigma}}}
\newcommand{\SR}[1]{{\ensuremath{\mathrm{#1}}}}
\newcommand{\BSR}[1]{{\ensuremath{\mathbf{#1}}}}
\newcommand{\composite}{{composite}}

%\newcommand{\alphat}{\ensuremath{\ensuremath{\alpha_{T}}}}
%\newcommand{\etmiss}{\ensuremath{\slashed{E}_T}}
%\newcommand{\pmiss}{\ensuremath{\slashed{p}}}
%\newcommand{\ptmiss}{\ensuremath{\slashed{p}_T}}
%\newcommand{\Ptmiss}{\ensuremath{{\slashed{\bf p}}_T}}
\def\Ptmiss{\ensuremath{\vec{E}_\mathrm{T}^{\mathrm{miss}}}}

\def\lsim{\mathrel{\rlap{\lower4pt\hbox{\hskip1pt$\sim$}}
    \raise1pt\hbox{$<$}}}                % less than or approx. symbol
\def\gsim{\mathrel{\rlap{\lower4pt\hbox{\hskip1pt$\sim$}}
    \raise1pt\hbox{$>$}}}                % greater than or approx. symbol

%\renewcommand{\thesubfigure}{\alpha{subfigure}}
%\makeatletter
%\renewcommand{\p@subfigure}{\arabic{figure}}
%\renewcommand{\thesubfigure}{\alph{subfigure}}
%\renewcommand{\@thesubfigure}{(\thesubfigure)}
%\makeatother

